LoyalDiffusion: A Diffusion Model Guarding Against Data Replication

Diffusion models have demonstrated significant potential in image generation. However, their ability to replicate training data presents a privacy risk, particularly when the training data includes confidential information. Existing mitigation strategies primarily focus on augmenting the training dataset, leaving the impact of diffusion model architecture under explored. In this paper, we address this gap by examining and mitigating the impact of the model structure, specifically the skip connections in the diffusion model's U-Net model. We first present our observation on a trade-off in the skip connections. While they enhance image generation quality, they also reinforce the memorization of training data, increasing the risk of replication. To address this, we propose a replication-aware U-Net (RAU-Net) architecture that incorporates information transfer blocks into skip connections that are less essential for image quality. Recognizing the potential impact of RAU-Net on generation quality, we further investigate and identify specific timesteps during which the impact on memorization is most pronounced. By applying RAU-Net selectively at these critical timesteps, we couple our novel diffusion model with a targeted training and inference strategy, forming a framework we refer to as LoyalDiffusion. Extensive experiments demonstrate that LoyalDiffusion outperforms the state-of-the-art replication mitigation method achieving a 48.63% reduction in replication while maintaining comparable image quality.

==> sec/2_related_works.tex <==
\section{Related Works}


\begin{figure*}[t]
      \centering
      \includegraphics[width=\textwidth]{sec/figure/Overview.png}
      \caption{Architecture of the proposed strategies to mitigate replication. Here, we show the skip connection group 3 \& 4 being modified to one single Conv 3×3 layer. GC\&DF represents generalized captioning and a dual fusion enhancement~\cite{}.}
      \label{fig:overview}
\end{figure*}


\subsection{Diffusion Models}

Denoising Diffusion Probabilistic Models (DDPMs)~\cite{ho2020denoising} have shown significant success in generative tasks~\cite{lugmayr2022repaint, ho2022video, lemercier2024diffusion}, which use a parameterized Markov chain to reverse a noise-adding process, reconstructing data from noise. However, their high computational complexity led to the development of Latent Diffusion Models (LDMs)~\cite{rombach2022high}, which reduce this cost by training in a compressed latent space. LDMs first encode images into a lower-dimensional latent space using an autoencoder, where a DDPM is then trained. Additionally, building on existing guidance techniques in diffusion models (DMs)~\cite{dhariwal2021diffusion, ho2022classifier}, LDMs employ cross-attention~\cite{vaswani2017attention} to enable multi-modal guidance by injecting conditional information at each timestep to better control generation. 

\subsection{Replication and mitigation strategies}
Despite their success, diffusion models are vulnerable to unintended memorization and replication of training data~\cite{somepalli2023diffusion, somepalli2023understanding, li2024mitigate, carlini2023extracting, duan2023diffusion}, which raises concerns about privacy and data security in sensitive applications.
Somepalli et al.~\cite{somepalli2023diffusion, somepalli2023understanding} introduce and define the concept of replication in diffusion models as the memorization of specific details from training images. Replication is largely driven by image duplication in the training data~\cite{somepalli2023understanding}. Furthermore, highly specific captions act as keys that retrieve specific data points from the model’s memory~\cite{somepalli2023understanding, li2024mitigate}. This issue is further intensified by smaller datasets, where limited diversity increases the likelihood of memorization~\cite{somepalli2023understanding}. 

Existing mitigation strategies focus mostly on optimizing training data. \cite{webster2023duplication, abbas2023semdedup} apply image deduplication to identify and remove both exact duplicates and semantically similar images. To generalize captions, Somepalli et al. propose methods including using multiple captions to training DMs (MC), adding Gaussian noise to text embeddings (GN), randomly replacing captions (RC), randomly replacing or adding tokens or words in captions (RT), repeating a random word in random location (CWR), and randomly adding a number to captions (RNA)~\cite{somepalli2023understanding}. Additionally, Li et al. introduce a generality score to quantify caption abstraction and use LLM~\cite{achiam2023gpt} to generalize captions, along with a dual-fusion technique that merges each training image with an external image-caption pair based on a set weighting, thereby reducing memorization risks. This approach focuses on a combination of caption generalization and image deduplication, thereby significantly reduces replication. Anti-Memorization Guidance (AMG)~\cite{chen2024towards} includes three guidance strategies, Despecification Guidance, Caption Deduplication Guidance, and Dissimilarity Guidance, all aiming at addressing memorization arising from image and caption duplication and over-specification. Wen et al.~\cite{wen2024detecting} suggest using perturbed prompt embeddings to minimize text-conditional prediction magnitude at diffusion inference, and screen out potential memorized pairs based on prediction magnitude during training. However, these data-centric strategies predominantly address replication externally, without examining the model’s internal mechanisms that contribute to memorization. %Moreover, differential privacy~\cite{dockhorn2022differentially, liu2023differentially} has also been applied to DMs, but it can degrade the model's output quality and reduce fidelity in generated images. 
Machine unlearning~\cite{bourtoule2021machine} is able to erase and remove specific content from the models and several studies have introduced it to mitigate replication~\cite{zhang2024forget, kumari2023ablating}. However, it can be computationally expensive and has potential to introduce new vulnerabilities. 

To address those shortcomings, in this paper, we propose a novel approach to mitigate replication by focusing on the diffusion model structure, specifically the UNet architecture and training strategy.
% offering an internal, structure-oriented solution to replication in diffusion models.

\subsection{UNet and skip connection}
To overcome optimization challenges in deep networks, ResNet~\cite{he2016deep} introduced skip connections, which add layers' input to their output. Skip connections effectively address the degradation problem by helping stabilize gradients during training and enhancing information flow across layers~\cite{xu2024development}.
%allowing deep neural networks to start converging even as the accuracy saturates~\cite{xu2024development}. 
Based on this property, skip connections have been applied to various UNet designs~\cite{ronneberger2015u, badrinarayanan2017segnet, zhou2019unet++, mao2016image}. UNet~\cite{ronneberger2015u} consists of an encoder, which downsamples to capture semantic information, and a decoder, which upsamples to reconstruct detailed outputs. Long skip connections link the encoder’s local details with the decoder’s broader contextual information, enhancing accuracy in tasks like pixel-level segmentation and object detection.

Due to these advantages, UNet serves as the backbone of DMs. However, while skip connections improve feature retention, they may also increase the risk of replication by enabling the diffusion model to memorize specific details from training data~\cite{wen2024detecting}.

% \label{sec:formatting}

% All text must be in a two-column format.
% The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% page.

% %-------------------------------------------------------------------------
% \subsection{Margins and page numbering}

% All printed material, including text, illustrations, and charts, must be kept
% within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
% high.
% %
% Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
% The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
% The \LaTeX\ template takes care of this when used properly.



% %-------------------------------------------------------------------------
% \subsection{Type style and fonts}

% Wherever Times is specified, Times Roman may also be used.
% If neither is available on your word processor, please use the font closest in
% appearance to Times to which you have access.

% MAIN TITLE.
% Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
% The title should be in Times 14-point, boldface type.
% Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
% do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
% Leave two blank lines after the title.

% AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
% and printed in Times 12-point, non-boldface type.
% This information is to be followed by two blank lines.

% The ABSTRACT and MAIN TEXT are to be in a two-column format.

% MAIN TEXT.
% Type main text in 10-point Times, single-spaced.
% Do NOT use double-spacing.
% All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% Make sure your text is fully justified---that is, flush left and flush right.
% Please do not place any additional blank lines between paragraphs.

% Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
% Short captions should be centred.

% \noindent Callouts should be 9-point Helvetica, non-boldface type.
% Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

% FIRST-ORDER HEADINGS.
% (For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

% SECOND-ORDER HEADINGS.
% (For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
% If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

% %-------------------------------------------------------------------------
% \subsection{Footnotes}

% Please use footnotes\footnote{This is what a footnote looks like.
% It often distracts the reader from the main flow of the argument.} sparingly.
% Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
% If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
% Use Times 8-point type, single-spaced.


% %-------------------------------------------------------------------------
% \subsection{Cross-references}

% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_preliminaries.tex <==
\section{Preliminaries}

\textbf{Problem Statement.} 
% \textbf{Notations.}
We refer to a pre-trained stable diffusion v2.1~\cite{} model as \emph{SD}, which is used as the baseline model for the rest of this paper. The %required training
fine-tuning dataset is typically formed with a large number of image-caption pairs, denoted as $D_{FT}=\{(x^{n}, y^{n})\}_{n=1}^N$, where $x^{n}$ is the $n$-th image, and $y^{n}$ is its corresponding caption. 
Fine-tuning a diffusion model involves two phases: the forward process and the training process. 
The forward process adds noise iteratively to each training image $x$ over $T$ timesteps, gradually transforming it into pure Gaussian noise. %$x_{T}$. 
We use $x_{t}$ and $\epsilon_t$ to denote the noisy input data and the noise added to the input at time step $t$, respectively.
In the training process, \emph{SD} learns to reverse this transformation, gradually denoising the noisy data to reconstruct the original input. Specifically,
%In the reverse process, we aim to gradually denoise $x_{T}$ back to $x_{0}$. 
a UNet parameterized by $\theta$ learns to estimate the noise $\epsilon_t$ %\epsilon_{\theta}(x_{t},t)$ 
added at timestep $t$, and \emph{SD} can then subtract the predicted noise from $x_t$ to iteratively refine the data. The loss function for training the UNet is as follows:
% \begin{equation}
%     L(\theta) = E_{\varepsilon, t}[\|\varepsilon - \varepsilon_{\theta}(x_{n}^{(t)}, t, y_{n})\|^2].
% \end{equation}
\begin{equation}
    L(\theta) = E_{\varepsilon, t}[\|\epsilon_t - \varepsilon_{\theta}(x_t, t, y)\|^2],
\end{equation}
where $\varepsilon_{\theta}(x_t, t, y)$ represents the noise predicted by the UNet for the noisy data $x_t$ at time step $t$ conditioned on the caption $y$.

As shown in Figure~\ref{}, UNet is a symmetric, encoder-decoder architecture with skip connections that play a critical role in diffusion models. 
Encoder path consists of multiple convolutional layers and cross attention blocks to do down sampling operations. For each down-sampling step $l$ in the encoder:
\begin{equation}
    h_{l} = down\_sampling(h_{l-1}),
\end{equation}
where $h_{l}$ is the feature map at layer $l$.
Bottleneck provides the lowest-level representation with maximum compression. Decoder path uses up sampling layers to expand back to the original resolution. For each up-sampling step $k$ in the decoder:
\begin{equation}
    u_{k} = up\_sampling(u_{k+1} \oplus h_{k}),
\end{equation}
where $u_{k}$  represents the feature map in the decoder path, $h_{k}$ is the corresponding encoder feature map passed via the skip connection, and $\oplus$ is concatenation operation.

The generative process is expressed as $g_{n} = SD(p_{n}, r)$, where $g_{n}$ represents the generated image, $p_{n}$ represents the corresponding caption, and $r$ represents the initial random noise. Building upon Somepalli et al.'s research~\cite{somepalli2023understanding}, $X=\{x_{n}\}_{n=1}^N$ and $G=\{g_{n}\}_{n=1}^N$ exist significant object-level copying, defined as replication. 

\textbf{Replication Score}
How to quantify data replication is complicated as it may refer to a diverse set of notions including object-level, semantic-level, and style-level replication. To simplify the evaluation process, we follow~\cite{somepalli2023understanding, somepalli2023diffusion} which focuses on object-level replication. In particular, in order for comparative analyses with existing research, we evaluate replication based on the metrics proposed by~\cite{somepalli2023understanding}. 
By calculating the feature map similarity between dataset $X$ and $G$, the probability density function of (PDF) of $S$ can be obtained as $pdf_{S}(S)$ and its cumulative distribution function (CDF) is $cdf_{S}(S<s)$, where random variable $S$ represents the similarity score. Since too many low-similarity images may distort the similarity of the entire dataset, only the top $5\%$ of the similarity distribution is taken into account. This threshold $R(X, G)\in{[0, 1]}$ is represented as the dataset replication score, defined as:
\begin{equation}
     P(S < R) = cdf_{S}(S < R) = 0.95.
\end{equation}
A higher value of $R(X, G)$ indicates a more pronounced degree of replication.

==> sec/5_approach.tex <==
\section{The Proposed LoyalDiffusion Framework}

Our approach to reducing replication in diffusion models, as shown in Figure \ref{fig:overview}, 
has three components. 
First, we introduce a replication-aware UNet(RAUNet), which replaces the UNet’s skip connections with more complex
%convolutional layers
information transfer blockers, mitigating the transference of direct features between the encoder and decoder of the model. Secondly, we propose a two-stages training strategy that applies the RAUNet only at higher timesteps, 
% where we hypothesize replication risks are greatest, 
where the impact on fidelity and quality of generation is minimal while still maintaining significant replication reduction,
using a standard UNet at lower timesteps to avoid fidelity of finer details being destroyed. 
Finally, we show how these techniques can be combined with generalized captioning and dual-fusion enhancement to further improve generalization and sample quality.

%\subsection{Observation}

\subsection{Replication-Aware UNet}

In diffusion models that use UNet architectures, skip connections play a crucial role in preserving spatial information by connecting corresponding layers of the encoder and decoder. Typically, these skip connections are identity functions that pass encoder features directly to the decoder.  We hypothesize that these direct transfer can lead to replication in the generated images. 
% We will show this under information theory perspective. 
% Let $h_{l}^t$ denote the encoder feature maps at layer $l$ at timestep $t$, which possess high entropy $H(h_{l}^t)$ due to the rich spatial details they encompass. The decoder feature maps from the previous layer are represented by $u_{l+1}^t$, with entropy $H(u_{l+1}^t)$. the input to the decoder at layer $l$ is obtained by concatenating the encoder and decoder features:
% \begin{equation}
%     u_{l}^t = h_{l}^t \oplus u_{l+1}^t.
% \end{equation}
% To simplify the analysis, we assume that $h_{l}^t$ and $u_{l+1}^t$ are independent, the entropy of the combined features is:
% \begin{equation}
%     H(u_{l}^t) = H(h_{l}^t \oplus u_{l+1}^t) = H(h_{l}^t) + H(u_{l+1}^t).
% \end{equation}
% By concatenating $h_{l}^t$ with $u_{l+1}^t$, the entropy $H(u_{l}^t)$ becomes higher than $H(u_{l+1}^t)$ alone, meaning decoder layers must process a vast amount of information, including potentially redundant or irrelevant details. This excessive information can overwhelm the decoder, causing it to replicate input patterns.

Skip connections in UNet architectures are designed to preserve spatial features from the encoder by passing them directly to the decoder, effectively bypassing the bottleneck layer~\cite{}. This direct transfer helps retain high-resolution details that might otherwise be lost during the encoding and decoding processes. However, the bypassing also means the decoder block relies less on the most compressed and abstract features from the bottleneck layer which
help reduce the reliance on specific features. 
By allowing unaltered feature maps to flow directly to the decoder, the network risks that these detailed inputs may dominate the abstracted, high-level representations.

As a result, the decoder can become overly dependent on these unaltered encoder features. Instead of learning to generate new content based on latent representations, the decoder might start copying details directly from the encoder—a "copy-paste" behavior. This mechanism impacts the information flow by allowing high-resolution details to take precedence, limiting the network's ability to learn general, abstract representations. This direct copying reduces the diversity and novelty of the generated content, making the model more prone to reproducing specific features from the training data rather than creating new, varied outputs.

% \textbf{Mitigation strategy}
% To mitigate replication, we have to reduce the entropy that decoder need to process. So we need to reduce $H(h_{l}^t)$ by using some operations $k$ on $h_{l}^t$ instead of not directly copying the features of the encoder to the decoder. The encoder features before they reach the decoder become $\hbar_{l}^t = k(h_{l}^t)$. $k$ need to act as a filter and feature transformation, reducing the entropy of the encoder features but transferring useful features: 
% \begin{equation}
%     H(\tilde{h}_{l}^t) = H(k(h_{l}^t) \leq H(h_{l}^t),
% \end{equation}
% since deterministic functions like convolutions cannot increase entropy. The total decder input entropy becomes:
% \begin{equation}
%     \begin{split}
%         H(\tilde{u}_{l}^t) &= H(\tilde{h}_{l}^t \oplus u_{l+1}^t) \\
%         &= H(\tilde{h}_{l}^t) + H(u_{l+1}^t) \leq H(h_{l}^t) + H(u_{l+1}^t)
%     \end{split}
% \end{equation}
% The total entropy is reduced compared to the case with identity skip connections. This simplification allows the decoder to process essential information more effectively, reducing the likelihood of replicating input patterns.

% To reduce the entropy of the encoder features $h_{l}^t$ before they are merged with the decoder features $u_{l+1}^t$, we explore various methods, including removing skip connection (RSK), max pooling (MP), convolutional layer (Conv), multiple convolutional layers (Multi-Conv), and attention layer (Att). Additionally, we investigate which skip connections have the most significant influence on replication by selectively change that skip connection to $k$.The experimental results and analysis will be shown in Section 5.
\textbf{Mitigation strategy:} To mitigate the replication caused by direct skip connections in UNet architectures, we propose several information transfer blockers applied to the skip connections.

\begin{enumerate}
    \item Removing Skip Connections (RSK): Eliminating skip connections entirely forces the decoder to rely only on the bottleneck's compressed representations, reducing replication risk. However, this may also lose important spatial information, potentially affecting image detail.
    \item Max Pooling (MP): Max pooling reduces the spatial dimensions of features in the skip connections, emphasizing prominent elements and condensing encoder information. It helps prevent the decoder from accessing detailed patterns, while still preserving essential spatial information.
    \item Convolutional Layer (Conv): Adding a convolutional layer to the skip connections allows the model to transform encoder features before passing them to the decoder, suppressing redundant patterns that could lead to replication. By adjusting the features, the convolutional layer helps balance the detailed information and the abstract representations.
    \item Multiple Convolutional Layers (Multi-Conv): Extending this idea with multiple convolutional layers offers deeper feature processing, creating complex abstractions to further reduce replication artifacts. However, this approach may increase computational costs and degrade image quality.
    % \item Attention Layer (Att): Adding an attention layer lets the model dynamically weigh the importance of different spatial features. It focuses on the most relevant parts, filtering out less significant details that could contribute to replication.
\end{enumerate}

To further understand which skip connections contribute most to replication artifacts, we propose to selectively modify specific skip connections rather than applying transformations uniformly across all of them. By experimenting with different configurations, such as transforming only the skip connections at certain layers, we can identify the stages in the network where replication is most pronounced.

\subsection{Two-stages Diffusion Training}

\begin{figure}[t]
      \centering
      \includegraphics[width=0.49\textwidth]{sec/figure/Similarity_CLIP_at_inference.png}
      \caption{Similarity between a training image and the generated image that replicates it and CLIP score calculating using the caption during the diffusion generating process.  It shows that similarity and CLIP score do not change too much during the early inference interval with large timesteps.}
      \label{fig:two-stage-approach}
\end{figure}

%Building upon our efforts to mitigate replication artifacts through entropy reduction in skip connections, 
We recognize that applying the RAU-Net uniformly across all timesteps in the diffusion process may negatively impact overall model performance. To address this, we propose a two-stages diffusion training approach that strategically applies RAU-Net only at 
% the most influential timesteps for replication or 
the least influential timesteps for generation quality, thereby balancing the trade-off between replication reduction and model fidelity.

As shown in Figure \ref{fig:two-stage-approach}, we analysis the behavior of generating process for a highly replicated generated image. We use pairwise similarity score to represent the quality of generated image and CLIP score~\cite{} to manage how well it matches the prompt.  The similarity increases most rapidly during the later timesteps, when $t$ is large, but is stable at early timesteps, which suggests that early timesteps are less important to image quality comparing with the later timesteps. The CLIP score curve almost show the same trend, remaining almost unchanged during early timesteps.
Intuitively, during these early timesteps, the noise level remains high, making it difficult for the model to capture detailed features that define the generated image quality or precise alignment with the prompt. At this stage, the model primarily operates in a generalized manner, with limited specificity, as the high noise overwhelms finer details from the training data. This observation suggests that these early timesteps are less critical for maintaining high-quality generation results. By strategically applying RAU-Net only during these high-noise, low-impact timesteps, we can minimize any potential adverse effects on generating quality while still benefiting from RAU-Net's replication reduction capabilities. 

On the other hand, during the early timesteps, the model begins by generating high-level information, such as object outlines and shapes, as shown in Figure \ref{fig:two-stage-approach}. These foundational elements establish the general direction of the subsequent generation process. Given that our study's replication score is based on object-level, we hypothesize that this high-level information generated in the early stages is a critical factor in replication.

% the model generates high-level information from complete noise, such as object outlines and shapes, which establish the general direction of the subsequent generation process. In contrast, the later timesteps refine detailed information. Since the replication score used in our study is based at the object-level, we hypothesize that the high-level information generated in the early stages plays a crucial role in replication, whereas subsequent detailed refinements have a limited impact.

% As shown in Figure \ref{fig:two-stage-approach}, the similarity between generated samples increases most rapidly during the initial timesteps, suggesting that replication primarily occurs at larger timesteps. Intuitively, during these early timesteps, when $t$ is large, the model generates high-level information from complete noise, such as object outlines and shapes, which establish the general direction of the subsequent generation process. In contrast, the later timesteps refine detailed information. Since the replication score used in our study is based at the object-level, we hypothesize that the high-level information generated in the early stages plays a crucial role in replication, whereas subsequent detailed refinements have a limited impact.

Based on these insights, we propose a two-stage training strategy with a predefined threshold timestep $\tau$. When $t > \tau$, the RAU-Net $U_{ra}$ is employed and only trained on noisy training samples within $t\in(\tau, T)$. For $t \leq \tau $, the standard U-Net $U_{st}$ is used and only trained on $t\in[\tau, T]$ training samples. 

Mathematically, the denoising process at each timestep $t$ can be defined as:
\begin{equation}
x_{t-1} = \begin{cases}
U_{\text{ra}}(x_t, t), & \text{if } t > \tau, \\
U_{\text{st}}(x_t, t), & \text{if } t \leq \tau,
\end{cases}
\end{equation}
where $x_{t}$ is the noisy image at timestep $t$.
During training, both U-Nets are optimized concurrently but each is responsible for different ranges of timesteps. 
% Specifically, $U_{\text{standard}}$ is trained on noisy images from $x_{0}$ to $x_{\tau}$, while $U_{\text{de-rep}}$ is trained on noisy images from $x_{\tau+1}$ to $x_{T}$. 
The total loss is the sum of the losses from both U-Nets:
\begin{equation}
L(\theta_{\text{st}}, \theta_{\text{ra}}) = L(\theta_{\text{st}}) + L(\theta_{\text{ra}})
\end{equation}

%In summary, this two-stage approach allows us to selectively apply the de-replicate UNet during the most critical timesteps, thereby minimizing adverse effects on overall model performance.

\subsection{Combining with Dataset Optimization}

To further enhance replication mitigation, we show our approach can be integrated with the state-of-the-art generalized caption and dual-fusion techniques~\cite{li2024mitigate}. Generalized captioning reduces replication by transforming specific captions into more generalized descriptions using a large language model~\cite{}, thereby encouraging the model to learn broad patterns instead of memorizing specific details. Dual-fusion further supports this by fusing a training image with another image from a different resource, using a weighted fusion of both the images and their captions. These approaches tend to diversify the training data, making it harder for the model to replicate exact training samples. Together with our LoyalDiffusion, this combination addresses replication from both data and model perspectives.

\subsection{Evaluating Replication using Bing Search}
To further evaluate replication, we utilize the Bing search engine to retrieve relevant images from the internet using the same prompts used during the inference phase, forming a new dataset named \textit{RepliBing}. This approach helps to find optimal comparisons for replication analysis. We aim to mitigate replication by ensuring that the generated images resemble real world images, as real world images are unlikely to be direct replications of one another. The internet image set represents a broad and diverse set of real world images, which closely align with the intended prompts, serving as an ideal reference. We calculate the replication score between the web image set and the training image set, referred to as the real world replication score $R_{real}$. As a result, we can view $R_{real}$ as a bottom line replication level that is acceptable in real world.

==> sec/6_experiments.tex <==
\section{Experiments}\label{sec:experiment}

\subsection{Setup}\label{sec:experiment_setup}
To evaluate our strategy, we fine-tune large pre-trained models on small datasets, as this approach tends to intensify data replication issues []. This worst-case scenario allows us to assess the limits of our approach in mitigating replication.

\textbf{Baseline:} We use Stable Diffusion [] as our baseline model, which is currently one of the state-of-the-art text-to-image generation models trained on the LAION dataset []. Stable Diffusion consists of: a text encoder, an image autoencoder, a diffusion module, and an image decoder. For our experiments, we fine-tune the Stable Diffusion v2.1 [] with $T=1000$, focusing specifically on the U-Net structure.

\textbf{Dataset:} For training, we randomly sample 10,000 instances from the LAION-2B [] dataset. Each instance contains an image paired with its corresponding caption, providing a diverse set of content covering various objects and contexts.

\textbf{Training and evaluation:} In our setup, all components except the U-Net are frozen during fine-tuning. We adopt most of the hyperparameters from [], including training for 100,000 iterations with a learning rate of $5e^{-6}$. For evaluation, we generate 10,000 images and use three primary metrics: the replication score R to quantify the extent of replication in generated samples, the Frechet Inception Distance (FID) [] to assess the quality and diversity of generated images, and the CLIP Score [] to evaluate the semantic similarity between generated images and their corresponding captions.

\textbf{Real world replication score:} We calculate the replication score between \textit{RepliBing} and the training image set, resulting in a replication score of $R_{real}=0.275$. It turn out that the replication score is not zero because even real-world images may share similar high-level structures or features, especially when generated from similar prompts.

% \textbf{Optimal replication score:} To further evaluate replication, we utilize the Bing search engine to retrieve relevant images from the internet using the same prompts used during the inference phase. This approach helps to find optimal comparisons for replication analysis. We aim to mitigate replication by ensuring that the generated images resemble real-world images, as real-world images are unlikely to be direct replications of one another. The internet image set represents a broad and diverse set of real-world images, which closely align with the intended prompts, serving as an ideal reference. We calculate the replication score between the web image set and the training image set, resulting in a replication score of $0.27543$, referred to as the optimal replication score $R_{opt}$. It turn out that the replication score is not zero because even real-world images may share similar high-level structures or features, especially when generated from similar prompts.

% \subsection{RAU-Net Results}
% The information transfer blockers we apply are set up as follows:

% (1) \textit{RSK}: Simply remove skip connection and concatenate feature map from last decoder with itself;

% (2) \textit{MP}: Max pooling with kernel size $2\times2$, followed by a \textit{MaxUnpool} that set all no-maximal values to $0$;

% (3) \textit{Conv}: A single convolutional layer with kernel size $3\times3$, without changing the output feature shape;

% (4) \textit{Multi-Conv}: $3$ Convolutional layers with kernel size $3\time3$, serving as downsampling, bootleneck, and upsampling. 

% We analyze the effectiveness of different information transfer blockers for reducing replication. In this evaluation, we applied each blocker uniformly to all skip connections within the U-Net. The results are shown in Table~\ref{tab:raunet-result-1}.

% \begin{table}[]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|ccccccc}
% \hline
%      & Opt     & Baseline & RSK     & MP      & Conv    & Multi-Conv & Att \\ \hline
% R$\downarrow$    & 0.275 & 0.617  & 0.232 & 0.581 & 0.186 & 0.194    & -   \\ \hline
% FID$\downarrow$  & -       & 18.01   & 127.73 & 19.65  & 200.37 & 234.50    & -   \\ \hline
% CLIP$\uparrow$ & -       & 0.313        & -       & -       & -       & -          & -   \\ \hline
% \end{tabular}%
% }
% \caption{}
% \label{tab:table-1}
% \end{table}

% \begin{table}[]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|ccccccc}
% \hline
%      & Real     & Baseline & RSK     & MP      & Conv    & Multi-Conv \\ \hline
% R$\downarrow$    & 0.275 & 0.617  & 0.232 & 0.581 & 0.186 & 0.194     \\ \hline
% FID$\downarrow$  & -       & 18.01   & 127.73 & 19.65  & 200.37 & 234.50    \\ \hline
% % CLIP$\uparrow$ & -       & 0.313        & -       & -       & -       & -         \\ \hline
% \end{tabular}%
% }
% \caption{}
% \label{tab:raunet-result-1}
% \end{table}

% These results indicate poor performance when applying a single operation uniformly across all skip connections. Specifically, the FID scores for \textit{Conv}, \textit{Multi-Conv}, and \textit{RSK} indicate significantly reduced image quality, disrupting the model's ability to generate high-quality outputs. This is likely due to the fact that different skip connections play varying roles in maintaining spatial information, and applying the same blocker across all of them disrupts this balance.

Given the poor outcomes, we decided to adjust our strategy by selectively modifying specific groups of skip connections within the U-Net, rather than applying uniform changes across all skip connections. In the standard U-Net architecture, there are four down-sampling blocks and four corresponding up-sampling blocks, each connected through skip connections. We consider these skip connections within each U-Net block pair as a group, resulting in four distinct groups. Each group captures different levels of feature information, from low-level details in the first group to higher-level semantic features in the deeper groups. By treating these skip connection groups independently, we can analyze how modifying each group impacts the model's ability to balance replication control and image quality. The results are summarized in Table \ref{tab:raunet-result-2}.

% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|c|c|cccc|cccc|ccccl|cccc}
% \hline
%         & opt     & baseline & \multicolumn{4}{c|}{RSK}             & \multicolumn{4}{c|}{MP}           & \multicolumn{5}{c|}{Conv}                      & \multicolumn{4}{c}{Multi-Conv}     \\ \hline
% Skip group & -       & -        & 1       & 2      & 3       & 4       & 1      & 2      & 3      & 4      & 1       & 2       & 3       & 4       & 3\&4   & 1      & 2      & 3       & 4      \\ \hline
% R$\downarrow$          & 0.275 & 0.617  & 0.570 & 0.583 & 0.601 & 0.621 & 0.614 & 0.608 & 0.602 & 0.617 & 0.450 & 0.561 & 0.444 & 0.628 & \textbf{0.386} & 0.537 & 0.582 & 0.511 & 0.620 \\ \hline
% FID$\downarrow$        & -       & 18.01   & 22.96  & 22.60 & 21.19  & 19.67  & 19.77 & 19.17 & 17.59 & 18.65 & 44.58  & 22.36  & 21.37  & 18.00  & \textbf{21.31} & 27.34 & 20.96 & 21.11  & 18.29 \\ \hline
% CLIP$\uparrow$       & -       & 0.313        & 0.307       & 0.304      & 0.306       & 0.313      & 0.313      & 0.314      & 0.314      & 0.314        & 0.287        & 0.301       & 0.290       & 0.314       &    0.304   & 0.302      & 0.306      & 0.298       & 0.313      \\ \hline
% \end{tabular}%
% }
% \caption{}
% \label{tab:raunet-result-2}
% \end{table*}


% \textbf{Analysis}
For \textit{RSK}, the modifications do not have a significant effect on replication control, with at most only a $7.52\%$ improvement in the replication score compared to the baseline, but costing FID increasing by $4.95$ and CLIP score reducing by $0.xx$. For \textit{MP}, although removing partial information in feature map doesn't destroy FID and CLIP score, the replication reduction is negligible, with only $2.43\%$ improvment. This suggests that limiting features on skip connections disrupts the flow of information necessary for high-quality reconstruction.
% , resulting in a trade-off that ultimately harms the model's generative capability.

For \textit{Conv}, modifying skip connection group 3 yielded the best result, with a $27.92\%$ improvement in the replication score, and only an increase of $3.36$ in FID and $0.xx$ in CLIP score. This indicates that modifying skip connections containing higher-level features with \textit{Conv} is effective in reducing replication. This may be due to group 3 containing higher-level feature information, which has a more significant impact on controlling replication compared to earlier groups that focus more on lower-level details.

Interestingly, modifying skip connection group 4 using a \textit{Conv} resulted in almost no change in both replication and FID. This suggests that the information carried by group 4 skip connections may not contribute significantly to replication issues. Given this finding, we experimented with modifying both group 3 and group 4 together. The result showed a replication score of $0.386$, further improving upon modifying only group 3 by $13.07\%$ and $37.44\%$ better than baseline, without increasing FID and CLIP score. This indicates that modifying both groups allows us to retain the quality of higher-level feature representations while reducing replication.

\textit{Multi-Conv} reduces replication less than CONV 
with almost the same FID and CLIP score. The reason for this may be multiple convolutional layers may lead to additional overfitting.

They key takeaway from this design exploration is that simply cutting off the skip connections may not be effective. Instead, it is crucial to transform the feature information in the skip connections into a different form, allowing the model to retain essential information while effectively mitigating replication.

\subsection{Two-Stage Training Results}
Building on the effective reduction of replication achieved by RAU-Net, which replaces skip connection groups 3 and 4 with \textit{Conv}, we selected this architecture for further experimentation.
% To evaluate a multi-stage training strategy, we employ both the standard U-Net $U_{st}$ and the RAU-Net $U_{ra}$ and a threshold timestep $\tau$.

To evaluate a two-stages training strategy, the standard U-Net $U_{st}$ is trained on timesteps $t \leq \tau$, while the RAU-Net $U_{ra}$ handles timesteps $t > \tau$.
% the alternative setup reverses this arrangement. This design aims to determine whether larger or smaller timesteps have a greater impact on replication. By understanding which stages each architecture performs best, we can improve the overall effectiveness of the denoising process. 
Then we apply different $\tau\in\{100, 300, 500, 700, 900\}$ and the results are shown in Table \ref{tab:two-stage-result_1}.
% and \ref{tab:two-stage-result_2}.

\begin{table}[]
\centering
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{c|ccccc}
\hline
t\_\{threshold\} & 100    & 300             & 500    & 700    & 900    \\ \hline
R$\downarrow$                & 0.373 & \textbf{0.378} & 0.453 & 0.558 & 0.606 \\ \hline
FID$\downarrow$              & 22.08 & \textbf{19.17} & 18.89 & 18.33 & 16.77 \\ \hline
CLIP$\uparrow$             & 0.290      & \textbf{0.301}               & 0.306      & 0.313      & 0.316      \\ \hline
\end{tabular}%
}
\caption{Results for switching different $\tau$, with $U_{st}$ for $t\leq \tau$ and $U_{ra}$ (\textit{Conv} on skip connection group 3 \& 4) for $t>\tau$.}
\label{tab:two-stage-result_1}
\end{table}


% \textbf{Analysis} 
From the results, we find that the best performance is achieved when training $U_{st}$ on timesteps $t \leq 300$ and the $U_{ra}$ on timesteps $t > 300$. This configuration results in an $38.74\%$ reduction in the replication score compared to the baseline model and an $2.07\%$ reduction compared to training without two-stages strategy. Additionally, this approach reduces the FID score by $2.14$ compared to using only the $U_{ra}$, and improves CLIP score by $0.xx$, indicating improved model generation ability.

% We also plotted the replication score and FID versus timesteps during inference to understand the impact on different stages, as shown in Figure x. These plots, comparing the baseline model, the de-replicate U-Net, and the best-performing multi-stage model, show that ...........


\subsection{Combining with Data Set Optimization}

\begin{figure}[t]
      \centering
      \includegraphics[width=\columnwidth]{sec/figure/mitigating_examples_2.pdf}
      \caption{Images in the first row are from training dataset that are replicated. Images in the second row are generated using fine-tuned baseline Stable Diffusion v2.1~\cite{rombach2022high}, which show obvious replication with training images. Images in the third row are generated by our best performance model, with much less content replicated with training images.}
      \label{fig:mitigating-examples}
\end{figure}

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|ccccccccccccccc}
\hline
       & Opt   & Baseline & \multicolumn{15}{c}{LoyalDiffusion + Generalized Captions + Dual-Fusion}                                                                                                                    \\ \hline
$w_{lat}$ & -     & -        & \multicolumn{5}{c|}{0.1}                                   & \multicolumn{5}{c|}{0.1}                                   & \multicolumn{5}{c}{0.1}               \\ \hline
$w_{emb}$ & -     & -        & \multicolumn{5}{c|}{0.1}                                   & \multicolumn{5}{c|}{0.3}                                   & \multicolumn{5}{c}{0.5}               \\ \hline
$\tau$      & -     & -        & 100   & 300   & 500   & 700   & \multicolumn{1}{c|}{900}   & 100   & 300   & 500   & 700   & \multicolumn{1}{c|}{900}   & 100   & 300   & 500   & 700   & 900   \\ \hline
R$\downarrow$      & 0.275 & 0.617    & 0.384 & 0.394 & 0.430 & 0.531 & \multicolumn{1}{c|}{0.562} & 0.341 & 0.351 & 0.363 & 0.443 & \multicolumn{1}{c|}{0.484} & 0.316 & \textbf{0.316} & 0.321 & 0.365 & 0.392 \\ \hline
FID$\downarrow$    & -     & 18.01    & 18.42 & 18.07 & 17.89 & 15.92 & \multicolumn{1}{c|}{14.79} & 21.03 & 18.15 & 18.42 & 17.22 & \multicolumn{1}{c|}{17.00} & 21.11 & \textbf{18.98} & 19.51 & 18.44 & 18.12 \\ \hline
CLIP$\uparrow$   & -     & 0.313        & 0.293     & 0.304     & 0.312     & 0.315     & \multicolumn{1}{c|}{0.316}     & 0.292     & 0.306     & 0.313     & 0.318     & \multicolumn{1}{c|}{0.318}     & 0.288     & \textbf{0.308}     & 0.313     & 0.318     & 0.319     \\ \hline
\end{tabular}%
}
\caption{}
\label{tab:result-with-GCDF}
\end{table*}

Building on previous work, we incorporate generalized captions (GC) and apply dual-fusion (DF) to further mitigate replication. For dual-fusion, we perform image fusion in the latent space using a weight $w_{lat} = 0.1$ and text fusion at the embedding level with $w_{emb} = 0.1, 0.3, 0.5$. 
% We explore the combination of these techniques with two main configurations: (1) using only the de-replicate U-Net, and (2) employing multi-stage training with the de-replicate U-Net. 
The experimental results are presented in Table X.

% \textbf{Analysis} 
The combination of GC\&DF with LoyalDiffusion significantly improves the performance. With $w_{lat}=0.1$, $w_{emb}=0.5$ and $\tau=300$, it achieves a reduction in replication of $48.78\%$ with only $0.97$ FID and $0.005$ CLIP score loss, comparing with baseline. Furthermore, even with a strict FID that should be almost same as baseline, our method can still achieve $43.11\%$ reduction of replication, with $w_{lat}=0.1$, $w_{emb}=0.3$ and $\tau=300$. These results support the claim that GC\&DF and our architectural modifications complement each other, 
GC\&DF mitigates replication from the data perspective, while our methods target the model structure itself. %Together, they work to reduce replication without negatively impacting model performance.

\subsection{Comparison with Prior-art}

We compare our approach with several prior-art methods designed to mitigate replication, including multiple captions (MC), Gaussian noise (GN), random caption replacement (RC), caption word repetition (CWR)
% , random token addition (RTA)
, Generalized Captions and Dual-Fusion Enhancement (GC\&DF).
% , and other state-of-the-art methods (placeholder for future methods). 
The results are shown in Table \ref{tab:compare-prior}. 
% Each method aims to address replication from different perspectives, either by modifying the input data or by changing the model architecture or training strategy. 
Specifically, our method outperforms the best prior-art method, GC\&DF~\cite{li2024mitigate}, by $24.58\%$, without significantly destroy FID.

\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cccccccccc}
\hline
 % & \begin{tabular}[c]{@{}c@{}}Base-\\ line\end{tabular} & MC~\cite{somepalli2023understanding}    & GN~\cite{somepalli2023understanding}    & RC~\cite{somepalli2023understanding}    & CWR~\cite{somepalli2023understanding}   & GC\&DF~\cite{li2024mitigate} & \begin{tabular}[c]{@{}c@{}}Ours w/o\\ GC\&DF\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ours w.\\ GC\&DF\end{tabular} \\ \hline
 & \begin{tabular}[c]{@{}c@{}}Base-\\ line\end{tabular} & \begin{tabular}[c]{@{}c@{}}MC\\ ~\cite{somepalli2023understanding}\end{tabular} & \begin{tabular}[c]{@{}c@{}}GN\\ ~\cite{somepalli2023understanding}\end{tabular} & \begin{tabular}[c]{@{}c@{}}RC\\ ~\cite{somepalli2023understanding}\end{tabular} & \begin{tabular}[c]{@{}c@{}}CWR\\ ~\cite{somepalli2023understanding}\end{tabular} & \begin{tabular}[c]{@{}c@{}}GC\&\\ DF~\cite{somepalli2023understanding}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ours w/o\\ GC\&DF\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ours w.\\ GC\&DF\end{tabular} \\ \hline
R$\downarrow$         & 0.617                                                & 0.420 & 0.596 & 0.565 & 0.614 & 0.419  & 0.378                                                     & \textbf{0.316}                                                    \\ \hline
FID$\downarrow$       & 18.01                                                & 16.83 & 19.50 & 15.98 & 16.73 & 17.16 & 19.17                                                     & 18.98                                                    \\ \hline
\end{tabular}%
}
\caption{Comparison with other prior works.}
\label{tab:compare-prior}
\end{table}
% \subsection{Deal with membership inference attacks}

\subsection{Visual Comparison}

We present a visual comparison to show the effectiveness of our approach in Figure~\ref{fig:mitigating-examples}, which includes original images from the training dataset, the most likely replicated image generated by the baseline model, and  our best-performing model. The comparison illustrates a significant reduction of replication.
% , demonstrating that our method effectively limits repetitive patterns in the generated outputs.

Additionally, our best-performing model achieves a replication score that is very close to the real world replication score $R_{real}$, indicating that our approach is highly effective in mitigating replication.


% \subsection{Analysis trade-off between R and FID}


